Tasty Burgers, Soggy Fries: Probing Aspect Robustness in Aspect-Based Sentiment Analysis

Aspect-based sentiment analysis (ABSA) aims to predict the sentiment towards a specific aspect in the text. However, existing ABSA test sets cannot be used to probe whether a model can distinguish the sentiment of the target aspect from the non-target aspects. To solve this problem, we develop a simple but effective approach to enrich ABSA test sets. Specifically, we generate new examples to disentangle the confounding sentiments of the non-target aspects from the target aspect's sentiment. Based on the SemEval 2014 dataset, we construct the Aspect Robustness Test Set (ARTS) as a comprehensive probe of the aspect robustness of ABSA models. Over 92% data of ARTS show high fluency and desired sentiment on all aspects by human evaluation. Using ARTS, we analyze the robustness of nine ABSA models, and observe, surprisingly, that their accuracy drops by up to 69.73%. We explore several ways to improve aspect robustness, and find that adversarial training can improve models' performance on ARTS by up to 32.85%. Our code and new test set are available at https://github.com/zhijing-jin/ARTS_TestSet

==> sec/tab_def_diff.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|lll|lll|lll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Laptop}     & \multicolumn{3}{c|}{Restaurant} & \multicolumn{3}{c}{MAMS}                                                  \\ \cmidrule(l){2-10} 
                         & \textsc{DelDiff}$^\dagger$ & \textsc{DelDiff} & change       & \textsc{DelDiff}$^\dagger$ & \textsc{DelDiff} &change         & \textsc{DelDiff}$^\dagger$ & \textsc{DelDiff} &change         \\ \midrule
MemNet                   & 35.62     & 38.36     & 7.69\%  & 39.73     & 46.58     & 17.24\% & 69.86     & 72.39     & 3.62\%  \\
AttLSTM               & 43.84     & 47.95     & 9.38\%  & 43.84     & 53.42     & 21.85\% & 66.56     & 66.67     & 0.17\%  \\ 
GatedCNN                     & 47.95     & 49.32     & 2.86\%  & 39.73     & 49.32     & 24.14\% & 65.13     & 67.33     & 3.38\%  \\ 
GCN                 & 47.95     & 60.27     & 25.69\% & 56.58     & 71.05     & 25.57\% & 77.67     & 77.34     & -0.42\% \\
TD-LSTM                 & 56.16     & 60.27     & 7.32\%  & 43.84     & 43.94     & 0.23\%  & 77.67    & 78.11     & 0.57\%  \\ 
CapsBERT             & 49.32     & 60.27     & 22.20\% & 71.71     & 73.68     & 2.75\%  & 84.05     & 81.96     & -2.49\% \\ 
BERT                & 67.12     & 68.49     & 2.04\%  & 50.68     & 58.90     & 16.22\% & 85.92     & 81.85     & -4.74\% \\ 
BERT-PT                  & 63.01     & 65.75     & 4.35\%  & 63.01     & 64.19     & 1.87\%  & 85.48     & 83.28     & -2.57\% \\ 
 \midrule
AVG & & &10.19\% & & &13.73\% & & &-0.31\%\\
\bottomrule
\end{tabular}%
}
\caption{Accuracy score on the adversarial test set by randomly deleting the aspect whose sentiment polarity is different with the target aspect. $^\dagger$ means the subset of the original test set.}
\label{tab:del_diff}
\end{table*}

==> sec/tab_mams.tex <==
\begin{table*}[!ht]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Model & \multicolumn{1}{c}{Entire Test} & \multicolumn{1}{c}{\textsc{RevTgt}} & \multicolumn{1}{c}{\textsc{RevNon}} &  \multicolumn{1}{c}{\textsc{AddDiff}} 
\\
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)}
\\
\hline 
\multicolumn{6}{l}{\textbf{\textit{Laptop Dataset}}} 
\\ 
GCAE & 65.67 $\rightarrow$ 10.34 (-55.33)$^\star$ & 75.11 $\rightarrow$ 24.03 (-51.08)$^\star$ & 84.44 $\rightarrow$ 78.52 (-5.92) & 65.67 $\rightarrow$ 44.98 (-20.69)$^\star$ 
\\
MemNet & 64.42 $\rightarrow$ 16.93 (-47.49)$^\star$ & 72.10 $\rightarrow$ 28.33 (-43.77)$^\star$ & 82.22 $\rightarrow$ 79.26 (-2.96) & 64.42 $\rightarrow$ 56.58 (-7.84)$^\star$ 
\\
ATAE-LSTM & 67.55 $\rightarrow$ 9.87 (-57.68)$^\star$ & 72.75 $\rightarrow$ 27.04 (-45.71)$^\star$ & 85.93 $\rightarrow$ 75.56 (-10.37)$^\star$ & 67.55 $\rightarrow$ 39.50 (-28.05)$^\star$ 
\\
TD-LSTM & 68.03 $\rightarrow$ 22.57 (-45.46)$^\star$ & 73.39 $\rightarrow$ 29.83 (-43.56)$^\star$ & 83.70 $\rightarrow$ 77.04 (-6.66) & 68.03 $\rightarrow$ 60.66 (-7.37)$^\star$ 
\\
ASGCN-DG & 72.41 $\rightarrow$ 19.91 (-52.50)$^\star$ & 78.33 $\rightarrow$ 35.62 (-42.71)$^\star$ & 88.89 $\rightarrow$ 74.81 (-14.08)$^\star$ & 72.41 $\rightarrow$ 52.51 (-19.90)$^\star$ 
\\
BERT-SENT & 73.04 $\rightarrow$ 17.40 (-55.65)$^\star$ & 78.76 $\rightarrow$ 59.44 (-19.32)$^\star$ & 88.15 $\rightarrow$ 42.22 (-45.93)$^\star$ & 73.04 $\rightarrow$ 34.64 (-38.40)$^\star$ 
\\
CapsNet-BERT & 76.80 $\rightarrow$ 25.86 (-50.94)$^\star$ & 80.90 $\rightarrow$ 57.30 (-23.60)$^\star$ & 90.37 $\rightarrow$ 50.37 (-40.00)$^\star$ & 76.80 $\rightarrow$ 45.14 (-31.66)$^\star$ 
\\
BERT-PAIR & 77.59 $\rightarrow$ 50.94 (-26.65)$^\star$ & 83.05 $\rightarrow$ 65.02 (-18.03)$^\star$ & 93.33 $\rightarrow$ 71.85 (-21.48)$^\star$ & 77.59 $\rightarrow$ 71.00 (-6.59)$^\star$ 
\\
BERT-PT & 78.53 $\rightarrow$ 53.29 (025.24)$^\star$ & 82.40 $\rightarrow$ 60.09 (-22.31)$^\star$ & 93.33 $\rightarrow$ 83.70 (-9.63)$^\star$ & 78.53 $\rightarrow$ 75.71 (-2.82) 
\\
\textbf{Average} &-46.33 &-34.45 & -17.45 & -18.15
\\ \hline

\multicolumn{6}{l}{\textbf{\textit{Restaurant Dataset}}} 
\\
GCAE &76.96 $\rightarrow$ 13.13 (-63.83)$^\star$& 85.11 $\rightarrow$ 23.17 (-61.94)$^\star$ & 87.84 $\rightarrow$ 72.75 (-15.09)$^\star$ & 76.96 $\rightarrow$ 55.00 (-21.96)$^\star$
\\
MemNet &75.18 $\rightarrow$ 21.52 (-53.66)$^\star$ & 80.73 $\rightarrow$ 27.54 (-53.19)$^\star$ & 84.46 $\rightarrow$ 73.65 (-10.81)$^\star$ & 75.18 $\rightarrow$ 60.71 (-14.47)$^\star$ 
\\
ATAE-LSTM &75.98 $\rightarrow$ 14.64 (-61.34)$^\star$ & 82.64 $\rightarrow$ 28.96 (-53.78)$^\star$ & 86.26 $\rightarrow$ 60.81 (-25.45)$^\star$ & 75.98 $\rightarrow$ 52.32 (-23.66)$^\star$
\\
TD-LSTM &78.12 $\rightarrow$ 30.18 (-47.94)$^\star$ & 85.24 $\rightarrow$ 34.99 (-50.35)$^\star$ & 88.51 $\rightarrow$ 75.68 (-12.83)$^\star$ & 78.12 $\rightarrow$ 70.18 (-7.94)$^\star$
\\
ASGCN-DG &77.86 $\rightarrow$ 24.73 (-53.13)$^\star$& 86.76 $\rightarrow$ 35.58 (-51.18)$^\star$ & 88.51 $\rightarrow$ 79.50 (-9.01)$^\star$ & 77.86 $\rightarrow$ 65.00 (-12.86)$^\star$ 
\\ 
BERT-SENT & 80.62 $\rightarrow$ 10.89 (-69.73)$^\star$ & 89.60 $\rightarrow$ 44.80 (-44.80)$^\star$ & 89.86 $\rightarrow$ 57.21 (-32.65)$^\star$ & 80.62 $\rightarrow$ 30.89 (-49.73)$^\star$ 
\\
CapsNet-BERT &83.66 $\rightarrow$ 55.36 (-28.30)$^\star$ & 89.73 $\rightarrow$ 71.99 (-17.84)$^\star$ & 90.99 $\rightarrow$ 73.20 (-17.79)$^\star$ & 83.66 $\rightarrow$ 77.86 (-5.80)$^\star$ 
\\
BERT-PAIR &83.04 $\rightarrow$ 54.82 (-28.22)$^\star$ & 90.07 $\rightarrow$ 63.00 (-27.07)$^\star$ & 91.44 $\rightarrow$ 83.33 (-8.11)$^\star$ & 83.04 $\rightarrow$ 79.20 (-3.84)$^\star$
\\
BERT-PT &86.70 $\rightarrow$ 59.29 (-27.41)$^\star$ & 92.20 $\rightarrow$ 72.81 (-19.39)$^\star$ & 92.57 $\rightarrow$ 81.76 (-10.81)$^\star$ & 86.70 $\rightarrow$ 80.27 (-6.43)$^\star$
\\
\textbf{Average} &-48.17 & -42.17 & -15.84 & -16.30
\\ \hline
\multicolumn{6}{l}{\textbf{\textit{MAMS Dataset}}} 
\\
GCAE & 66.02 $\rightarrow$ 32.93(-33.09)$^\star$   & 60.58 $\rightarrow$ 23.83 -36.75$^\star$ & 55.47 $\rightarrow$ 53.73 (-1.74) & 66.02 $\rightarrow$ 57.19 (-8.83)$^\star$ 
\\
MemNet & 70.51 $\rightarrow$ 37.80(-32.71)$^\star$ & 62.36 $\rightarrow$ 27.25 (-35.11)$^\star$ & 61.19 $\rightarrow$ 54.98 (-6.21) & 70.51 $\rightarrow$ 65.08 (-5.43)
\\
ATAE-LSTM & 67.14 $\rightarrow$ 39.76 (-27.38) $^\star$& 57.16 $\rightarrow$ 29.02 (-28.14)$^\star$ & 52.49 $\rightarrow$ 49.25 (-3.24) & 67.14 $\rightarrow$ 60.93 (-6.21)$^\star$ 
\\
TD-LSTM & 77.62 $\rightarrow$ 49.25 (-28.37)$^\star$ & 69.46 $\rightarrow$ 31.69 (-37.77)$^\star$ & 70.40 $\rightarrow$ 71.64 (1.24) & 77.62 $\rightarrow$ 76.57 (-1.05) 
\\
ASGCN-DG & 76.95 $\rightarrow$ 47.80 (-29.15)$^\star$ & 74.52 $\rightarrow$ 38.78 (-35.74)$^\star$ & 73.63 $\rightarrow$ 70.65 (-2.98) & 76.95 $\rightarrow$ 74.40 (-2.55) 
\\
BERT-SENT & 49.25 $\rightarrow$ 10.48 (-38.77)$^\star$ & 44.49 $\rightarrow$ 32.45 (-12.04)$^\star$ & 50.00 $\rightarrow$ 45.52 (-4.48) & 49.25 $\rightarrow$ 30.76 (-18.49)$^\star$
\\
CapsNet-BERT & 83.38 $\rightarrow$ 60.17 (-23.21) $^\star$ & 79.59 $\rightarrow$ 49.30 (-30.29)$^\star$ & 78.36 $\rightarrow$ 76.12 (-2.24) & 83.38 $\rightarrow$ 83.08 (-0.30) 
\\
BERT-PAIR & 84.51 $\rightarrow$ 61.38 (-23.13) $^\star$ & 80.61 $\rightarrow$ 49.18 (-31.43)$^\star$ & 77.36 $\rightarrow$ 76.87 (-0.49) & 84.51 $\rightarrow$ 83.01 (-1.50) 
\\
BERT-PT & 85.10 $\rightarrow$ 64.37 (-20.73) $^\star$ & 82.89 $\rightarrow$ 55.01 (-27.88)$^\star$ & 81.34 $\rightarrow$ 78.86 (-2.48) & 85.10 $\rightarrow$ 83.68 (-1.42)
\\
\textbf{Average} &-28.05 &-30.57 & -2.51 &-5.09
\\
\bottomrule
\end{tabular}
}
\caption{The accuracy score of different models on four adversarials of Laptop, Restaurant, and MAMS datasets. $\dagger$ means the performance on original testset subsets, and $\Delta$ represents a percentage decline. $\Delta\text{AVG}$ means the average percentage of decrease on four adversarial datasets. $\ast$ indicates the improvement over the adverserial dataset is statistically significant (Welch's $t$-test $p < 0.05$).}
\label{tab:adv-results}
\end{table*}

==> sec/table89_old.tex <==
\begin{table*}[!ht]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Model & \multicolumn{1}{c}{Entire Test} & \multicolumn{1}{c}{\textsc{RevTgt}} & \multicolumn{1}{c}{\textsc{RevNon}} &  \multicolumn{1}{c}{\textsc{AddDiff}} 
\\
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)}
\\
\hline 
\multicolumn{6}{l}{\textbf{\textit{Laptop Dataset}}} 
\\ 
GCAE & 65.67 $\rightarrow$ 40.76 (-24.91)$^\star$ & 75.11 $\rightarrow$ 24.03 (-51.08)$^\star$ & 84.44 $\rightarrow$ 78.52 (-5.92) & 65.67 $\rightarrow$ 44.98 (-20.69)$^\star$ 
\\
MemNet & 64.42 $\rightarrow$ 48.43 (-15.99)$^\star$ & 72.10 $\rightarrow$ 28.33 (-43.77)$^\star$ & 82.22 $\rightarrow$ 79.26 (-2.96) & 64.42 $\rightarrow$ 56.58 (-7.84)$^\star$ 
\\
ATAE-LSTM & 67.55 $\rightarrow$ 38.82 (-28.73)$^\star$ & 72.75 $\rightarrow$ 27.04 (-45.71)$^\star$ & 85.93 $\rightarrow$ 75.56 (-10.37)$^\star$ & 67.55 $\rightarrow$ 39.50 (-28.05)$^\star$ 
\\
TD-LSTM & 68.03 $\rightarrow$ 50.85 (-17.18)$^\star$ & 73.39 $\rightarrow$ 29.83 (-43.56)$^\star$ & 83.70 $\rightarrow$ 77.04 (-6.66) & 68.03 $\rightarrow$ 60.66 (-7.37)$^\star$ 
\\
ASGCN-DG & 72.41 $\rightarrow$ 48.59 (-23.82)$^\star$ & 78.33 $\rightarrow$ 35.62 (-42.71)$^\star$ & 88.89 $\rightarrow$ 74.81 (-14.08)$^\star$ & 72.41 $\rightarrow$ 52.51 (-19.90)$^\star$ 
\\
BERT-SENT & 73.04 $\rightarrow$ 44.79 (-28.25)$^\star$ & 78.76 $\rightarrow$ 59.44 (-19.32)$^\star$ & 88.15 $\rightarrow$ 42.22 (-45.93)$^\star$ & 73.04 $\rightarrow$ 34.64 (-38.40)$^\star$ 
\\
CapsNet-BERT & 76.80 $\rightarrow$ 50.36 (-26.44)$^\star$ & 80.90 $\rightarrow$ 57.30 (-23.60)$^\star$ & 90.37 $\rightarrow$ 50.37 (-40.00)$^\star$ & 76.80 $\rightarrow$ 45.14 (-31.66)$^\star$ 
\\
BERT-PAIR & 77.59 $\rightarrow$ 68.85 (-8.74)$^\star$ & 83.05 $\rightarrow$ 65.02 (-18.03)$^\star$ & 93.33 $\rightarrow$ 71.85 (-21.48)$^\star$ & 77.59 $\rightarrow$ 71.00 (-6.59)$^\star$ 
\\
BERT-PT & 78.53 $\rightarrow$ 70.70 (-7.83)$^\star$ & 82.40 $\rightarrow$ 60.09 (-22.31)$^\star$ & 93.33 $\rightarrow$ 83.70 (-9.63)$^\star$ & 78.53 $\rightarrow$ 75.71 (-2.82) 
\\
\textbf{Average} &-20.21 &-34.45 & -17.45 & -18.15
\\ \hline

\multicolumn{6}{l}{\textbf{\textit{Restaurant Dataset}}} 
\\
GCAE &76.96 $\rightarrow$ 47.10 (-29.86)$^\star$& 85.11 $\rightarrow$ 23.17 (-61.94)$^\star$ & 87.84 $\rightarrow$ 72.75 (-15.09)$^\star$ & 76.96 $\rightarrow$ 55.00 (-21.96)$^\star$
\\
MemNet &75.18 $\rightarrow$ 51.40 (-23.78)$^\star$ & 80.73 $\rightarrow$ 27.54 (-53.19)$^\star$ & 84.46 $\rightarrow$ 73.65 (-10.81)$^\star$ & 75.18 $\rightarrow$ 60.71 (-14.47)$^\star$ 
\\
ATAE-LSTM &75.98 $\rightarrow$ 45.77 (-30.21)$^\star$ & 82.64 $\rightarrow$ 28.96 (-53.78)$^\star$ & 86.26 $\rightarrow$ 60.81 (-25.45)$^\star$ & 75.98 $\rightarrow$ 52.32 (-23.66)$^\star$
\\
TD-LSTM &78.12 $\rightarrow$ 58.84 (-19.28)$^\star$ & 85.24 $\rightarrow$ 34.99 (-50.35)$^\star$ & 88.51 $\rightarrow$ 75.68 (-12.83)$^\star$ & 78.12 $\rightarrow$ 70.18 (-7.94)$^\star$
\\
ASGCN-DG &77.86 $\rightarrow$ 57.34 (-20.52)$^\star$& 86.76 $\rightarrow$ 35.58 (-51.18)$^\star$ & 88.51 $\rightarrow$ 79.50 (-9.01)$^\star$ & 77.86 $\rightarrow$ 65.00 (-12.86)$^\star$ 
\\ 
BERT-SENT & 80.62 $\rightarrow$ 40.62 (-40.00)$^\star$ & 89.60 $\rightarrow$ 44.80 (-44.80)$^\star$ & 89.86 $\rightarrow$ 57.21 (-32.65)$^\star$ & 80.62 $\rightarrow$ 30.89 (-49.73)$^\star$ 
\\
CapsNet-BERT &83.66 $\rightarrow$ 75.15 (-8.51)$^\star$ & 89.73 $\rightarrow$ 71.99 (-17.84)$^\star$ & 90.99 $\rightarrow$ 73.20 (-17.79)$^\star$ & 83.66 $\rightarrow$ 77.86 (-5.80)$^\star$ 
\\
BERT-PAIR &83.04 $\rightarrow$ 74.27 (-8.77)$^\star$ & 90.07 $\rightarrow$ 63.00 (-27.07)$^\star$ & 91.44 $\rightarrow$ 83.33 (-8.11)$^\star$ & 83.04 $\rightarrow$ 79.20 (-3.84)$^\star$
\\
BERT-PT &86.70 $\rightarrow$ 77.93 (-8.77)$^\star$ & 92.20 $\rightarrow$ 72.81 (-19.39)$^\star$ & 92.57 $\rightarrow$ 81.76 (-10.81)$^\star$ & 86.70 $\rightarrow$ 80.27 (-6.43)$^\star$
\\
\textbf{Average} &-21.08 & -42.17 & -15.84 & -16.30
\\ \hline
\multicolumn{6}{l}{\textbf{\textit{MAMS Dataset}}} 
\\
GCAE & 66.02 $\rightarrow$ 53.15(-12.87)$^\star$   & 60.58 $\rightarrow$ 23.83 -36.75$^\star$ & 55.47 $\rightarrow$ 53.73 (-1.74) & 66.02 $\rightarrow$ 57.19 (-8.83)$^\star$ 
\\
MemNet & 70.51 $\rightarrow$ 57.44(-13.07)$^\star$ & 62.36 $\rightarrow$ 27.25 (-35.11)$^\star$ & 61.19 $\rightarrow$ 54.98 (-6.21) & 70.51 $\rightarrow$ 65.08 (-5.43)
\\
ATAE-LSTM & 67.14 $\rightarrow$ 55.32 (-11.82) $^\star$& 57.16 $\rightarrow$ 29.02 (-28.14)$^\star$ & 52.49 $\rightarrow$ 49.25 (-3.24) & 67.14 $\rightarrow$ 60.93 (-6.21)$^\star$ 
\\
TD-LSTM & 77.62 $\rightarrow$67.25 (-10.37)$^\star$ & 69.46 $\rightarrow$ 31.69 (-37.77)$^\star$ & 70.40 $\rightarrow$ 71.64 (1.24) & 77.62 $\rightarrow$ 76.57 (-1.05) 
\\
ASGCN-DG & 76.95 $\rightarrow$ 67.62 (-9.33)$^\star$ & 74.52 $\rightarrow$ 38.78 (-35.74)$^\star$ & 73.63 $\rightarrow$ 70.65 (-2.98) & 76.95 $\rightarrow$ 74.40 (-2.55) 
\\
BERT-SENT & 49.25 $\rightarrow$ 39.50 (-9.75)$^\star$ & 44.49 $\rightarrow$ 32.45 (-12.04)$^\star$ & 50.00 $\rightarrow$ 45.52 (-4.48) & 49.25 $\rightarrow$ 30.76 (-18.49)$^\star$
\\
CapsNet-BERT & 83.38 $\rightarrow$ 75.67 (-7.71) $^\star$ & 79.59 $\rightarrow$ 49.30 (-30.29)$^\star$ & 78.36 $\rightarrow$ 76.12 (-2.24) & 83.38 $\rightarrow$ 83.08 (-0.30) 
\\
BERT-PAIR & 84.51 $\rightarrow$ 75.98 (-8.53) $^\star$ & 80.61 $\rightarrow$ 49.18 (-31.43)$^\star$ & 77.36 $\rightarrow$ 76.87 (-0.49) & 84.51 $\rightarrow$ 83.01 (-1.50) 
\\
BERT-PT & 85.10 $\rightarrow$ 77.82 (-7.28) $^\star$ & 82.89 $\rightarrow$ 55.01 (-27.88)$^\star$ & 81.34 $\rightarrow$ 78.86 (-2.48) & 85.10 $\rightarrow$ 83.68 (-1.42)
\\
\textbf{Average} &-10.08 &-30.57 & -2.51 &-5.09
\\
\bottomrule
\end{tabular}
}
\caption{The accuracy score of different models on four adversarials of Laptop, Restaurant, and MAMS datasets. $\dagger$ means the performance on original testset subsets, and $\Delta$ represents a percentage decline. $\Delta\text{AVG}$ means the average percentage of decrease on four adversarial datasets. $\ast$ indicates the improvement over the adverserial dataset is statistically significant (Welch's $t$-test $p < 0.05$).}
\label{tab:adv-results}
\end{table*}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc|ccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{5}{c|}{Laptop}                               & \multicolumn{5}{c}{Restaurant}        \\
\multicolumn{1}{c}{} &
  O$\rightarrow$O &
  O$\rightarrow$A &
  A$\rightarrow$A &
  O$\rightarrow$A(u) &
  A$\rightarrow$A(u) &
  O$\rightarrow$O &
  O$\rightarrow$A &
  A$\rightarrow$A &
  O$\rightarrow$A(u) &
  A$\rightarrow$A(u) 
\\ \hline
GCAE                                        & 65.67                     & 49.28 & 65.42 & 10.34 & 41.85 & 76.96 & 56.57 & 67.39 & 13.13 & 37.50 \\
MemNet                                      & 64.42                     & 53.86 & 58.28 & 16.93 & 31.82 & 75.18 & 58.98 & 64.05 & 21.52 & 37.95 \\
ATAE-LSTM                                   & 67.55                     & 48.59 & 63.35 & 9.87  & 42.63 & 75.98 & 55.35 & 71.73 & 14.64 & 48.66 \\
TD-LSTM                                     & 68.03                     & 56.69 & 71.02 & 22.57 & 54.86 & 78.12 & 64.96 & 79.52 & 30.18 & 62.76 \\
ASGCN-DG                                    & 72.41                     & 56.69 & 73.42 & 19.91 & 56.43 & 77.86 & 63.85 & 80.08 & 24.73 & 61.52 \\
BERT-SENT                                   & 73.04                     & 54.40 & 73.95 & 17.40 & 53.92 & 80.62 & 53.31 & 75.07 & 10.89 & 45.80 \\
CapsNet-BERT                                & 76.80                     & 59.46 & 76.51 & 25.86 & 61.23 & 83.66 & 77.79 & 87.22 & 55.36 & 75.80 \\
BERT-PAIR                                   & 77.59                     & 71.82 & 77.09 & 50.94 & 65.67 & 83.04 & 77.05 & 86.52 & 54.82 & 74.82 \\
BERT-PT                                     & 78.53 & 73.36 & 77.78 & 53.29 & 66.93 & 86.70 & 80.71 & 86.91 & 59.29 & 74.64 \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:data_augmentation}
\end{table*}



==> sec/table8_old.tex <==
\begin{table*}[!ht]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Model & \multicolumn{1}{c}{Entire Test} & \multicolumn{1}{c}{\textsc{RevTgt}} & \multicolumn{1}{c}{\textsc{RevNon}} &  \multicolumn{1}{c}{\textsc{AddDiff}} 
\\
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)} 
& \multicolumn{1}{c}{before$\rightarrow$after (relat. effect)}
\\
\hline 
\multicolumn{5}{l}{\textbf{\textit{Laptop Dataset}}} 
\\ 
GCAE & 65.67 $\rightarrow$ 10.34 (-55.33)$^\star$ & 75.11 $\rightarrow$ 24.03 (-51.08)$^\star$ & 84.44 $\rightarrow$ 78.52 (-5.92) & 65.67 $\rightarrow$ 44.98 (-20.69)$^\star$ 
\\
MemNet & 64.42 $\rightarrow$ 16.93 (-47.49)$^\star$ & 72.10 $\rightarrow$ 28.33 (-43.77)$^\star$ & 82.22 $\rightarrow$ 79.26 (-2.96) & 64.42 $\rightarrow$ 56.58 (-7.84)$^\star$ 
\\
ATAE-LSTM & 67.55 $\rightarrow$ 9.87 (-57.68)$^\star$ & 72.75 $\rightarrow$ 27.04 (-45.71)$^\star$ & 85.93 $\rightarrow$ 75.56 (-10.37)$^\star$ & 67.55 $\rightarrow$ 39.50 (-28.05)$^\star$ 
\\
TD-LSTM & 68.03 $\rightarrow$ 22.57 (-45.46)$^\star$ & 73.39 $\rightarrow$ 29.83 (-43.56)$^\star$ & 83.70 $\rightarrow$ 77.04 (-6.66) & 68.03 $\rightarrow$ 60.66 (-7.37)$^\star$ 
\\
ASGCN-DG & 72.41 $\rightarrow$ 19.91 (-52.50)$^\star$ & 78.33 $\rightarrow$ 35.62 (-42.71)$^\star$ & 88.89 $\rightarrow$ 74.81 (-14.08)$^\star$ & 72.41 $\rightarrow$ 52.51 (-19.90)$^\star$ 
\\
BERT-SENT & 73.04 $\rightarrow$ 17.40 (-55.65)$^\star$ & 78.76 $\rightarrow$ 59.44 (-19.32)$^\star$ & 88.15 $\rightarrow$ 42.22 (-45.93)$^\star$ & 73.04 $\rightarrow$ 34.64 (-38.40)$^\star$ 
\\
CapsNet-BERT & 76.80 $\rightarrow$ 25.86 (-50.94)$^\star$ & 80.90 $\rightarrow$ 57.30 (-23.60)$^\star$ & 90.37 $\rightarrow$ 50.37 (-40.00)$^\star$ & 76.80 $\rightarrow$ 45.14 (-31.66)$^\star$ 
\\
BERT-PAIR & 77.59 $\rightarrow$ 50.94 (-26.65)$^\star$ & 83.05 $\rightarrow$ 65.02 (-18.03)$^\star$ & 93.33 $\rightarrow$ 71.85 (-21.48)$^\star$ & 77.59 $\rightarrow$ 71.00 (-6.59)$^\star$ 
\\
BERT-PT & 78.53 $\rightarrow$ 53.29 (025.24)$^\star$ & 82.40 $\rightarrow$ 60.09 (-22.31)$^\star$ & 93.33 $\rightarrow$ 83.70 (-9.63)$^\star$ & 78.53 $\rightarrow$ 75.71 (-2.82) 
\\
\textbf{Average} &-46.33 &-34.45 & -17.45 & -18.15
\\ \hline

\multicolumn{5}{l}{\textbf{\textit{Restaurant Dataset}}} 
\\
GCAE &76.96 $\rightarrow$ 13.13 (-63.83)$^\star$& 85.11 $\rightarrow$ 23.17 (-61.94)$^\star$ & 87.84 $\rightarrow$ 72.75 (-15.09)$^\star$ & 76.96 $\rightarrow$ 55.00 (-21.96)$^\star$
\\
MemNet &75.18 $\rightarrow$ 21.52 (-53.66)$^\star$ & 80.73 $\rightarrow$ 27.54 (-53.19)$^\star$ & 84.46 $\rightarrow$ 73.65 (-10.81)$^\star$ & 75.18 $\rightarrow$ 60.71 (-14.47)$^\star$ 
\\
ATAE-LSTM &75.98 $\rightarrow$ 14.64 (-61.34)$^\star$ & 82.64 $\rightarrow$ 28.96 (-53.78)$^\star$ & 86.26 $\rightarrow$ 60.81 (-25.45)$^\star$ & 75.98 $\rightarrow$ 52.32 (-23.66)$^\star$
\\
TD-LSTM &78.12 $\rightarrow$ 30.18 (-47.94)$^\star$ & 85.24 $\rightarrow$ 34.99 (-50.35)$^\star$ & 88.51 $\rightarrow$ 75.68 (-12.83)$^\star$ & 78.12 $\rightarrow$ 70.18 (-7.94)$^\star$
\\
ASGCN-DG &77.86 $\rightarrow$ 24.73 (-53.13)$^\star$& 86.76 $\rightarrow$ 35.58 (-51.18)$^\star$ & 88.51 $\rightarrow$ 79.50 (-9.01)$^\star$ & 77.86 $\rightarrow$ 65.00 (-12.86)$^\star$ 
\\ 
BERT-SENT & 80.62 $\rightarrow$ 10.89 (-69.73)$^\star$ & 89.60 $\rightarrow$ 44.80 (-44.80)$^\star$ & 89.86 $\rightarrow$ 57.21 (-32.65)$^\star$ & 80.62 $\rightarrow$ 30.89 (-49.73)$^\star$ 
\\
CapsNet-BERT &83.66 $\rightarrow$ 55.36 (-28.30)$^\star$ & 89.73 $\rightarrow$ 71.99 (-17.84)$^\star$ & 90.99 $\rightarrow$ 73.20 (-17.79)$^\star$ & 83.66 $\rightarrow$ 77.86 (-5.80)$^\star$ 
\\
BERT-PAIR &83.04 $\rightarrow$ 54.82 (-28.22)$^\star$ & 90.07 $\rightarrow$ 63.00 (-27.07)$^\star$ & 91.44 $\rightarrow$ 83.33 (-8.11)$^\star$ & 83.04 $\rightarrow$ 79.20 (-3.84)$^\star$
\\
BERT-PT &86.70 $\rightarrow$ 59.29 (-27.41)$^\star$ & 92.20 $\rightarrow$ 72.81 (-19.39)$^\star$ & 92.57 $\rightarrow$ 81.76 (-10.81)$^\star$ & 86.70 $\rightarrow$ 80.27 (-6.43)$^\star$
\\
\textbf{Average} &-48.17 & -42.17 & -15.84 & -16.30
\\ 
\bottomrule
\end{tabular}
}
\caption{The accuracy score of different models on four adversarials of Laptop, Restaurant, and MAMS datasets. $\dagger$ means the performance on original testset subsets, and $\Delta$ represents a percentage decline. $\Delta\text{AVG}$ means the average percentage of decrease on four adversarial datasets. $\ast$ indicates the improvement over the adverserial dataset is statistically significant (Welch's $t$-test $p < 0.05$).}
\label{tab:adv-results}
\end{table*}
